Coanda Flow Characterization on Base Bleed Configurations Using Global Stability Analysis

Base pressure control is often employed on drag reduction design, but the interaction of the jet with the base region flow topology can generate undesired or uncontrolled flow configurations. The ejected flow can drive pressure bifurcations at the trailing edge, that without a correct optimization can affect the aerodynamic performance of the system. The purpose of this work is to fully understand the physical mechanisms related with the use of injected base bleed employing global stability analysis and adjoint methodologies. Moreover, the results of the sensitivity analysis are used to identify the regions more receptive to passive and active flow control methodologies. This work has a particular relevance in turbine research, where coolant flow is ejected at the trailing edge to ensure an adequate thermal protection of the blade and the downstream turbine stages.

==> flow_control.tex <==
Controlling the flow downstream a turbine blade is one of the major challenges nowadays, as secondary flows drive most of the losses in this area. With the information extracted from this numerical analysis, we aim to show the capabilities of stability analysis based flow control. For this we propose two ways of action, based on passive and active flow control. The first is based on the modification or addition of geometry to the existent one in order to mitigate the instability, in this case to force a symmetric base bleed flow regardless the intensity of the jet. The second is however more complex, as we will be looking at the control of the flow at the base region by direct actuation on it. In order to obtain more information that could be used to guide the different flow control methods, a sensitivity analysis over selected configurations is computed. 

\subsection{Passive flow control}
The control of the instability for a supersonic flow configuration with a straight trailing edge is analyzed here. Being this the one firstly detected, and with more possible detrimental effects downstream the blade due to the alteration of the shock wave system\cite{Martinez-Cava2018}, this case was chosen as a test scenario for the neutralization of the instability. A small control cylinder of diameter $0.1h$ was placed at the location most sensitive to passive control, and tested for those base bleed mass flows for which the bifurcation was known to appear. The presence of the cylinder neutralized the instability and kept a constant symmetric state downstream the base region, as shown on Fig. RT. As a consequence of the presence of the cylinder, the flow was deflected towards both sides, impinging on the shear layers and strengthening the shock waves present at the trailing edge shock system. However, these changes remained symmetric and constant, in opposition to what was observed when the base bleed flow changed its direction due to the instability and impinged in just one of the shear layers.


\subsection{Active flow control}
\subsubsection{Synthetic jet actuation}
To take advantage of the \textit{Coanda} effect that takes place on a rounded trailing edge, one would like to be able to control the direction of the deflection of the base bleed flow when the global stability arises. This would mean being able to generate a \textit{Coanda} deflection when needed, and also to be able to swap the jet direction in a easy and efficient way. This was achieved here by the use of the so-called synthetic jets, based on zero-net mass flow actuators\cite{Kral1997NumericalActuators}. 

A synthetic jet can be modelled as a zero-net mass flow actuation, that generates flow blowing or suction of very small mass flows in an harmonic way. This particular boundary condition is already implemented in the DLR TAU-code, and has been tested against industrial cases showing a robust and consistent behavior. In this research, two actuators were placed symmetrically at the end of the injection channel of a rounded trailing edge, at the exact location predicted by the sensitivity analysis on Section \ref{sec-sensitivity}. The two actuators acted periodically at a given frequency, but with a phase difference of 180 degrees, with a maximum mass flow intensity of $C_q=XX$.

Different actuating frequencies were tested for subsonic and supersonic configurations, to evaluate the effects of active control on the global instability. All the tests showed a controlled change in the flow direction when the synthetic jet was applied, perfectly matching the frequency of the change of the flow direction with the frequency of the synthetic jets actuation. The combined effect of blowing/suction in opposite sides of the trailing edge, will push/pull the base bleed jet towards the side where suction was present, remaining there without changes until the synthetic jet was activated again in the opposite way. Results are shown on Fig HH, where the base bleed flow angle was plotted against time, together with the mass flow rates of the actuators. 

As the synthetic jet were applied at the region of maximum sensitivity, each actuation generates not only an obvious effect on the jet flow, but also a drift on the behavior of the instability. To probe the scope of the effects, the actuators were tested for a subsonic configuration where the instability is present but it is stable (base bleed intensity of $C_q=0.21$), meaning that no base bleed flow deflection is naturally present. The application of the synthetic jets awakes the instability, and an oscillating change in direction is generated during the time the actuators are present. Each alteration of the direction of the base bleed flow will imply the generation of a vortex that will travel downstream, recovering the flow afterwards the steady state present before the change of direction.

The change of direction of the base bleed flow has an increasing impact on the flow topology when the flow speed becomes supersonic, as shown on Section \ref{sec:flow-sup}. At low frequency actuation, the base region flow has time to adapt and find a steady position as the downstream shocks adapt to the changes generated by the change in the jet direction, and the detached vortex travels downstream from the base region. However, higher frequencies provoke the next change in the jet direction when the flow has not yet adapted to the new configuration, eventually generating a vortex shedding with frequency X times the frequency of the actuation. The effects near the airfoil are strong, but however downstream the effects seem to have a minor impact on the main trailing edge shock wave. POST PROCESSING REQUIRED. The change in flow direction of the base bleed jet responds perfectly to the actuating frequency, showing that localized feedback at the regions of maximum sensitivity can control the steady instability related with the \textit{Coanda} effect at the trailing edge.

\subsection{Pulsating base bleed flow}
On the pursue of base region flow control, previous attempts for manipulating the flow downstream were carried out by the application of pulsating base bleed flow\cite{Saavedra2017,Saracoglu2012}. The application of this methodology here aims to take advantage of the previous flow characterization, with available information about the blowing rates that will produce higher values of base pressure, and presumably a \textit{Coanda} effect apparition at the injection walls.

CONTAR ESTO TRAS HACER POSTPROCESO
